Agentic Path Maps: Exposing an Agent's Traversal Through the Garden of Forking Paths

When an AI agent executes an underspecified task, it embeds choices that may contradict unarticulated user context and preferences. However, interrupting the user for clarification on all such decisions is untenable. How might agents communicate impactful, but unexplored, paths to the user after execution? To investigate, we first distill a design space for communicating alternative paths, supporting the generation of new systems and structuring dimensions of future study. We then measure the impact of one vital design space dimension on user comprehension: the number of alternatives displayed. Through a user study (n=48) in the data analysis domain, we find that participants rarely consider alternative paths of their own volition, but AI overreliance reduces when alternative paths are visualized for them. By revealing paths the agent did not take, we demonstrate how users can better interpret results and incorporate personal context.

==> tables/design_space.tex <==
\makeatletter
\@ifundefined{dsdim}{\newlength{\dsdim}}{}
\@ifundefined{dsunit}{\newlength{\dsunit}}{}
\@ifundefined{dsrowh}{\newlength{\dsrowh}}{}
\@ifundefined{dsgap}{\newlength{\dsgap}}{}
\@ifundefined{dsvskip}{\newlength{\dsvskip}}{}
\@ifundefined{dscatw}{\newlength{\dscatw}}{}
\@ifundefined{dsrad}{\newlength{\dsrad}}{}
\@ifundefined{dsrule}{\newlength{\dsrule}}{}
\@ifundefined{dsiw}{\newlength{\dsiw}}{}
\@ifundefined{dsih}{\newlength{\dsih}}{}
\@ifundefined{dsbx}{\newsavebox{\dsbx}}{}
\providecommand{\dsn}[1]{\strip@pt\dimexpr#1\relax}
\makeatother

\setlength{\dsgap}{6pt}
\setlength{\dscatw}{13pt}
\setlength{\dsvskip}{3pt}
\setlength{\dsrad}{3.5pt}
\setlength{\dsrule}{0.8pt}
\providecommand{\dsfill}{black!12}

\providecommand{\Description}[1]{}
\providecommand{\dssetup}{%
  \settowidth{\dsdim}{\small Visualizations}%
  \setlength{\dsunit}{\dimexpr(\linewidth-\dsdim-\dscatw-12pt)/12\relax}%
  \setlength{\dsrowh}{13pt}%
  \setlength{\aboverulesep}{2pt}%
  \setlength{\belowrulesep}{2pt}%
  \setlength{\fboxsep}{2pt}}
\providecommand{\dsh}[1]{\global\setlength{\dsrowh}{#1}}

\providecommand{\dsdashh}[1]{%
  \hbox to #1{\cleaders\hbox to 4pt{\rule{2.4pt}{\dsrule}\hfil}\hfil}}
\providecommand{\dsdashv}[1]{%
  \vbox to #1{\cleaders\vbox to 4pt{\hbox{\rule{\dsrule}{2.4pt}}\vfil}\vfil}}

% rounded rectangle: #1 width, #2 height, #3 mode (0 fill, 1 outline, 2 dashed)
\providecommand{\dsRR}[3]{%
  \begingroup
  \setlength{\unitlength}{1pt}%
  \edef\dsRn{\dsn{\dsrad}}\edef\dsDn{\dsn{2\dsrad}}%
  \edef\dsEn{\dsn{0.5\dsrule+\dsrad}}%
  \begin{picture}(0,0)
    {\color{\dsfill}%
     \put(\dsRn,0){\rule{\dimexpr#1-2\dsrad\relax}{#2}}%
     \put(0,\dsRn){\rule{#1}{\dimexpr#2-2\dsrad\relax}}%
     \put(\dsRn,\dsRn){\circle*{\dsDn}}%
     \put(\dsn{#1-\dsrad},\dsRn){\circle*{\dsDn}}%
     \put(\dsRn,\dsn{#2-\dsrad}){\circle*{\dsDn}}%
     \put(\dsn{#1-\dsrad},\dsn{#2-\dsrad}){\circle*{\dsDn}}}%
    \ifnum#3>0
      \ifdim\dsrule<0.6pt\thinlines\else\thicklines\fi
      \put(\dsEn,\dsEn){\oval(\dsDn,\dsDn)[bl]}%
      \put(\dsn{#1-0.5\dsrule-\dsrad},\dsEn){\oval(\dsDn,\dsDn)[br]}%
      \put(\dsEn,\dsn{#2-0.5\dsrule-\dsrad}){\oval(\dsDn,\dsDn)[tl]}%
      \put(\dsn{#1-0.5\dsrule-\dsrad},\dsn{#2-0.5\dsrule-\dsrad}){\oval(\dsDn,\dsDn)[tr]}%
      \ifnum#3=1
        \put(\dsEn,0){\rule{\dimexpr#1-\dsrule-2\dsrad\relax}{\dsrule}}%
        \put(\dsEn,\dsn{#2-\dsrule}){\rule{\dimexpr#1-\dsrule-2\dsrad\relax}{\dsrule}}%
        \put(0,\dsEn){\rule{\dsrule}{\dimexpr#2-\dsrule-2\dsrad\relax}}%
        \put(\dsn{#1-\dsrule},\dsEn){\rule{\dsrule}{\dimexpr#2-\dsrule-2\dsrad\relax}}%
      \else
        \put(\dsEn,0){\dsdashh{\dimexpr#1-\dsrule-2\dsrad\relax}}%
        \put(\dsEn,\dsn{#2-\dsrule}){\dsdashh{\dimexpr#1-\dsrule-2\dsrad\relax}}%
        \put(0,\dsEn){\dsdashv{\dimexpr#2-\dsrule-2\dsrad\relax}}%
        \put(\dsn{#1-\dsrule},\dsEn){\dsdashv{\dimexpr#2-\dsrule-2\dsrad\relax}}%
      \fi
    \fi
  \end{picture}%
  \endgroup}

\providecommand{\dsslot}[2]{\makebox[#1\dsunit]{#2}}
\providecommand{\dstext}[2]{%
  \parbox[b][\dimexpr\dsrowh+2\fboxsep\relax][c]{\dimexpr#1\dsunit-\dsgap-2\fboxsep\relax}{%
    \linespread{0.9}\selectfont\centering #2}}
\providecommand{\dsmark}[3]{%
  \dsslot{#1}{\raisebox{-0.5\dimexpr\dsrowh+2\fboxsep\relax}{%
    \rlap{\dsRR{\dimexpr#1\dsunit-\dsgap\relax}{\dimexpr\dsrowh+2\fboxsep\relax}{#2}}%
    \hspace{\fboxsep}\dstext{#1}{#3}\hspace{\fboxsep}}}}

\providecommand{\dsH}{\dimexpr\dsrowh+2\fboxsep\relax}
% one shaded background spanning a run of adjacent shaded cells
\providecommand{\dsrun}[2]{\multicolumn{#1}{@{}c@{}}{%
  \rlap{\kern0.5\dsgap\raisebox{-0.5\dsH}{%
    \dsRR{\dimexpr#1\dsunit-\dsgap\relax}{\dsH}{0}}}#2}}
% a segment inside a run: span, mode (0 none, 1 outline, 2 dashed), text
\providecommand{\dsseg}[3]{%
  \dsslot{#1}{\raisebox{-0.5\dsH}{%
    \ifnum#2>0\relax\rlap{\dsRR{\dimexpr#1\dsunit-\dsgap\relax}{\dsH}{#2}}\fi
    \hspace{\fboxsep}\dstext{#1}{#3}\hspace{\fboxsep}}}}
\providecommand{\dsplain}[2]{\multicolumn{#1}{@{}c@{}}{%
  \dsslot{#1}{\raisebox{-0.5\dimexpr\dsrowh+2\fboxsep\relax}{%
    \hspace{\fboxsep}\dstext{#1}{#2}\hspace{\fboxsep}}}}}
\providecommand{\dsgrey}[2]{\multicolumn{#1}{@{}c@{}}{\dsmark{#1}{0}{#2}}}
\providecommand{\dspick}[2]{\multicolumn{#1}{@{}c@{}}{\dsmark{#1}{1}{#2}}}
\providecommand{\dspart}[2]{\multicolumn{#1}{@{}c@{}}{\dsmark{#1}{2}{#2}}}

% several alternatives sharing one box
\providecommand{\dsit}[2]{\parbox[c]{#1\linewidth}{\centering #2}}
\providecommand{\dstwo}[2]{\dsit{0.5}{#1}\dsit{0.5}{#2}}

\providecommand{\dsrow}[1]{%
  \raisebox{-0.5\dsH}{\parbox[b][\dsH][c]{\dsdim}{\raggedright #1}}}
\providecommand{\dssub}[1]{\\[0.5pt]{\footnotesize\itshape #1}}
\providecommand{\dsinline}[2]{%
  \sbox{\dsbx}{#2}%
  \setlength{\dsiw}{\dimexpr\wd\dsbx+5pt\relax}%
  \setlength{\dsih}{\dimexpr\ht\dsbx+\dp\dsbx+3.4pt\relax}%
  \begingroup\setlength{\dsrad}{2pt}\setlength{\dsrule}{0.4pt}%
  \raisebox{\dimexpr-\dp\dsbx-1.7pt\relax}{\rlap{\dsRR{\dsiw}{\dsih}{#1}}}%
  \endgroup
  \hspace{2.5pt}\usebox{\dsbx}\hspace{2.5pt}}
\providecommand{\dsgi}[1]{\dsinline{0}{#1}}
\providecommand{\dsoi}[1]{\dsinline{1}{#1}}
\providecommand{\dssep}{\hspace{2.5pt}}
% #1 = \dsh value of the row below, #2 = category label
\providecommand{\dscat}[2]{%
  \makebox[\dscatw]{\smash{%
    \raisebox{-0.5\dimexpr#1+2\fboxsep+4.4pt\relax}{%
      \raisebox{-0.5\height}{\rotatebox{90}{\footnotesize\bfseries #2}}}}}}
\providecommand{\dssplit}{\cmidrule(l){2-14}}
\providecommand{\dspre}{\dssetup\centering\small
  \setlength{\tabcolsep}{0pt}\renewcommand{\arraystretch}{1}}

\begin{table*}[t]
\dspre
\caption{Design space dimensions. Our design space for Agentic Path Maps has eight
dimensions in four categories: goals, initiative, content, and display. The space draws from ten related domains, so grey highlighting
indicates options specifically relevant for Agentic Path Maps. Black outlines situate our empirical study's stimulus within the design space, with the 
dotted outline around the \textbf{quantity} dimension we manipulate. In the actor row, A is agent, MI is mixed-initiative, U
is user, and I is inherent.}
\label{tab:design_space}
\Description{A design space table with category labels at the left, dimensions in the middle, and alternatives across each row. Goals groups Objectives and Structure, Initiative groups Actor and Timing, Content groups Quantity and Explanations, and Display groups Visualizations and Interactions. Solid outlines select Building understanding, Hierarchical decisions, Once, Path details, Decision sensitivity, specification curve, and Elicit details. In the Actor row, outlines select agent for Generating multiples and inherent for Determining granularity and Determining quantity. A shared dotted outline encloses All and Samples in the Quantity row. Gray backgrounds mark relevant alternatives. In the Actor row, though, these backgrounds apply to individual actor labels.
}

\begin{tabular}{@{}c@{\hspace{4pt}}l@{\hspace{8pt}}*{12}{@{}c@{}}@{}}
\toprule
& \textbf{Dimension} & \multicolumn{12}{c}{\textbf{Alternatives}}\\
\midrule
\dscat{13pt}{Goals}
  & \dsh{21pt}\dsrow{Objectives}
  & \dsrun{6}{\dsseg{3}{1}{Building understanding}%
              \dsseg{3}{0}{Integrating user perspective}}
  & \dsplain{3}{Improving task performance}
  & \dsplain{3}{Fostering creativity}\\
\dssplit
  & \dsh{13pt}\dsrow{Structure}
  & \dsplain{4}{Outcome set}
  & \dsrun{8}{\dsseg{4}{0}{Independent decisions}%
              \dsseg{4}{1}{Hierarchical decisions}}\\
\midrule
\dscat{13pt}{Initiative}
  & \dsh{30pt}\dsrow{Actor}
  & \dsplain{3}{Generating multiples\dssub{\dsoi{A}\dssep MI\dssep U}}
  & \dsplain{3}{Selecting multiples\dssub{A\dssep\dsgi{MI}\dssep\dsgi{U}}}
  & \dsplain{2}{Requesting more\dssub{A\dssep MI\dssep U}}
  & \dsplain{2}{Determining granularity\dssub{\dsgi{A}\dssep\dsgi{MI}\dssep\dsgi{U}\dssep\dsoi{I}}}
  & \dsplain{2}{Determining quantity\dssub{\dsgi{A}\dssep\dsgi{MI}\dssep\dsgi{U}\dssep\dsoi{I}}}\\
\dssplit
  & \dsh{13pt}\dsrow{Timing}
  & \dspick{3}{Once}
  & \dsplain{3}{Iterative sequence}
  & \dsplain{3}{Linear sequence}
  & \dsplain{3}{On demand}\\
\midrule
\dscat{21pt}{Content}
  & \dsh{13pt}\dsrow{Quantity}
  & \dspart{6}{\dstwo{All}{Samples}}
  & \dsplain{3}{Current step}
  & \dsgrey{3}{No outcomes}\\
\dssplit
  & \dsh{21pt}\dsrow{Explanations}
  & \dsrun{12}{\dsseg{2}{0}{Preferred choice}%
               \dsseg{2}{1}{Path details}%
               \dsseg{2}{0}{Highlight differences}%
               \dsseg{2}{1}{Decision sensitivity}%
               \dsseg{2}{0}{Performance metrics}%
               \dsseg{2}{0}{Trend aggregations}}\\
\midrule
\dscat{13pt}{Display}
  & \dsh{21pt}\dsrow{Visualizations}
  & \dsplain{6}{Collection\dssub{moodboard $\cdot$ text list}}
  & \dsgrey{6}{Dependency\dssub{trees/graphs $\cdot$ text $\cdot$ \dsoi{specification curve} $\cdot$ scatterplot}}\\
\dssplit
  & \dsh{13pt}\dsrow{Interactions}
  & \dsrun{10}{\dsseg{3}{0}{Integrate perspectives}%
               \dsseg{2}{0}{Navigate}%
               \dsseg{2}{0}{Aggregate}%
               \dsseg{3}{1}{Elicit details}}
  & \dsplain{2}{Request more}\\
\bottomrule
\end{tabular}
\end{table*}
